An Improved QFT-Based Quantum Comparator and Extended Modular Arithmetic Using One Ancilla Qubit

Quantum comparators and modular arithmetic are fundamental in many quantum algorithms. Current research mainly focuses on operations between two quantum states. However, various applications, such as integer factorization, optimization, option pricing, and risk analysis, commonly require one of the inputs to be classical. It requires many ancillary qubits, especially when subsequent computations are involved. In this paper, we propose a quantum-classical comparator based on the quantum Fourier transform (QFT). Then we extend it to compare two quantum integers and modular arithmetic. Proposed operators only require one ancilla qubit, which is optimal for qubit resources. We analyze limitations in the current modular addition circuit and develop it to process arbitrary quantum states in the entire $n$-qubit space. The proposed algorithms reduce computing resources and make them valuable for Noisy Intermediate-Scale Quantum (NISQ) computers.

==> 2.2_shor.tex <==
本章首先介绍量子算术运算、量子傅里叶变换及其应用、量子相位估计。其中量子傅里叶变换有很多的应用，如可以实现常数模四则运算，具体见\S \ref{sub:2.2.2}，量子傅里叶变换可以进一步实现量子相位估计，具体见\S \ref{sub:2.2.3}。量子模运算和量子傅里叶变换均是Shor实现的基本组件，最后\S \ref{sub:2.2.4} 节介绍Shor算法以及应用。


\subsection{量子算术运算}

在某些应用中，量子计算机中需要实现基本的四则运算。本节主要介绍量子算术基本组件的实现基本原理，包括加减乘除量子线路、模四则运算量子线路，并结合QPanda介绍相关接口的具体实现。


\subsubsection{基于UMA的算术运算}\label{sub:2.2.1}

\textbf{量子加法器}

目前，量子加法器有多种实现方法，最初的实现思想是将被加数$a,b$作为二进制展开，分别按位加并不断处理进位信息，即基于UMA实现的量子加法器。此种方法的实现主要包括两种子量子线路模块MAJ和UMA，作用分别是获得当前二进制位的进位数值和当前二进制位的结果数值。

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/addmau.jpg}
	\caption{基于UMA和MAJ的加法器}
	\label{fig:addmau}
\end{figure}


MAJ量子线路的输入分别为前一位的进位值$c_i$、当前位的两个待加值$a_i,b_i$，输出为$a_i+c_i \bmod 2$，$a_i+b_i\bmod 2$和当前位进位值$c_{i+1}$。

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/maj.jpg}
	\caption{MAJ的输入输出}
	\label{fig:maj}
\end{figure}


\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=MAJ代码实现,
label=code:maj
]{code/2.2/MAJ.py}

MAJ模块是为了实现获得进位，我们想要得到进位$c_{i+1}$，也就是要从$a_i+b_i+c_i$出发，判断$(a_i+b_i+c_i)/2$。在待加值中任选一个数$a_i$对进位情况进行如下枚举，
\begin{equation}
	\begin{split}
		a_i=0, \ & c_i=[(a_i+b_i)\bmod 2]*[(a_i+c_i)\bmod 2]\\
		a_i=1, \  & c_i=([(a_i+b_i)\bmod 2]*[(a_i+c_i)\bmod 2]+1)\bmod 2 
	\end{split}
\end{equation}
因此，只需要考察$a_i,[(a_i+b_i)\bmod 2]*[(a_i+c_i)\bmod 2]$就可以判断进位情况。从现有的量子逻辑门出发，制备量子态$a_i, (a_i+b_i)\bmod 2, (a_i+c_i)\bmod 2$，即可以准确判断出进位的情况。可以使用CNOT门来完成模2加法得到$(a_i+b_i)\bmod 2, (a_i+c_i)\bmod 2$，使用Toffoli门完成$a$ 与$[[(a_i+b_i)\bmod 2]*[(a_i+c_i)\bmod 2]$ 的异或运算。

UMA量子线路的输入分别为$a_i+c_i \bmod 2$， $a_i+b_i \bmod 2$和当前位进位值$c_{i+1}$，输出为$c_i$，$a_i+b_i+c_i \bmod 2=s_i$ 和$a_i$。
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/uma.jpg}
	\caption{UMA的输入输出}
	\label{fig:uma}
\end{figure}

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=UMA代码实现,
label=code:uma
]{code/2.2/UMA.py}

UMA模块是为了实现获得当前位结果，我们想要得到当前位$s_i$,也就是要得到$(a_i+b_i+c_i)\bmod 2$。通过与MAJ所用的完全相反的TOffoli门由$c_{i+1}$得到$a_i$，然后利用与MAJ所用的相反的CNOT变换得到$c_i$，综合已有的$a_i+b_i \bmod 2$，于是可以通过简单的CNOT门得到$(a_i+b_i+c_i)\bmod 2$。

在QPanda中加法器的接口函数如下：
\begin{itemize}
	\item QAdder(adder1,adder2,c,iscarry)
	\item QAdderIgnoreCarry(adder1,adder2,c)
	\item QAdd(adder1,adder2,k)
\end{itemize}
前两种接口函数的区别是是否保留进位，但都只支持正数加法。参数中adder1与adder2为执行加法的比特且格式完全一致，c为辅助比特。
第三种加法器接口函数是带符号的加法器，是基于量子减法器实现的。待加数添加了符号位，相应的辅助比特也从1-2个单比特变为一个adder1.size()+2比特。
加法的输出比特都是adder1，其他非进位比特不变。

第一个接口QAdder的量子线路设计如下所示，借助MAJ和UMA对adder1和adder2不断按位做亦或和进位计算：
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=QAddded的具体线路实现,
label=code:qadder
]{code/2.2/qadder.py}


\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=QAdder接口的测试,
label=code:textqadder
]{code/2.2/textqadder.py}

\begin{exercise}
	结合QAdder量子线路，构造QAdderIgnoreCarry加法器（不保留进位）。
\end{exercise}


\textbf{量子减法器}

基础的加法器只支持非负整数的加法。对于小数要求输入的被加数$a$和$b$必须小数点位置相同，小数点对齐后整体长度相同。
对于带符号变换的量子加法，则需要追加辅助比特用于记录符号位。任给两个目标量子态$A,B$，对第二个量子态$B$进行特定的补码操作，然后转换为$A-B=A+(-B)$，此处的$-B$并不以符号位取反的方式实现。
该特定的补码操作为：符号位为正则不变，符号位为负需要按位取反后再加1。因此需要一个额外的辅助比特来控制是否进行求补码的操作。具体补码的量子线路设计如所示。
量子减法器实质上就是量子加法器的带符号版本。

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=符号位为负的补码操作,
label=code:qcomplement
]{code/2.2/qcomplement.py}


在QPanda中减法器（带符号的加法器）的接口函数如下：
\begin{itemize}
	\item QSub(a,b,k)
\end{itemize}
与带符号的加法器相同，两个待减数的量子比特最高位为符号位，辅助比特k.size()=a.size()+2。
减法的输出比特是a，其他比特不变。下面给出加法的线路实现代码与具体测试，对于a-b小于0时，测量得到的最高位为1。

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=量子减法线路与测试,
label=code:qsub
]{code/2.2/qsub.py}

\begin{exercise}
	分析QAdder逆操作实现的减法和QSub实现减法的区别。
\end{exercise}

\textbf{量子乘法法器}

量子乘法器是基于加法器完成的。计算
\begin{equation}
	x*y=\sum_{i=0}^{n}2^{i}x_{i}y=x_{0}y+2(x_{1}y+2(x_{2}y+\cdots+2(x_{n-2}y+2(x_{n-1}y)))\cdots),
\end{equation}
选择乘数$y$作为受控比特，选择乘数$x$以二进制展开逐位作为控制比特，将受控加法器的运算结果累加到辅助比特中。每完成一次$x$控制的受控加法就将乘数$y$左移一位并在末位补零。
于是把通过受控加法输出的数值在辅助比特中累加起来，得到乘法结果。具体线路实现代码如下：

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=量子减法线路与测试,
label=code:qmul
]{code/2.2/qmultiplier.py}

在QPanda中乘法器的接口函数主要有两个：
\begin{itemize}
	\item QMultiplier(a,b,k,d)
	\item QMul(a,b,k,d)
\end{itemize}
两个接口函数的输入待乘量子比特都包含符号位，但只有QMul支持带符号的乘法运算。
相应的，QMultiplier中，辅助比特k.size()=a.size()+1，结果比特d.size()=2*a.size()。
QMul中，辅助比特k.size()=a.size()，结果比特d.size()=2*a.size()-1。
乘法的输出比特都是d，其他比特不变。如果等长的输入比特a和b存在小数点，那么在输出比特d中的小数点位置坐标为输入比特中的2倍。

下面给出接口QMultiplier的计算测试：
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=量子乘法的计算示例,
label=code:multext
]{code/2.2/multext.py}

\begin{exercise}
	结合 QMultiplier和QSub的量子线路，撰写带符号的乘法量子线路。
\end{exercise}

\textbf{量子除法器}

在经典计算计算机中，计算除法是非常容易的，其中最经典的辗转相除法可以计算商和余数，基本思想可以理解为每次将被除数减去除数，多次做减法后直到余数为0或者余数小于除数。
所以，本书的量子除法器是基于量子减法器完成的，通过执行减法后被除数的符号位是否改变来完成大小比较，并决定除法是否终止。被除数减去除数时，商结果加1。每完成一次减法后，重新进行被除数与除数的大小比较，直至除尽或者达到预设精度。因此还需要额外追加一个存储精度参数的辅助比特。下面介绍一般除法返回商和余数的代码\ref{code:qdiv}：
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=量子除法的一种代码实现,
label=code:qdiv
]{code/2.2/qdiver.py}


在QPanda中除法法器的接口函数如下：
\begin{itemize}
	\item QDivider(a,b,c,k,t)
	\item QDivider(a,b,c,k,f,s)
	\item QDiv(a,b,c,k,t)
	\item QDiv(a,b,c,k,f,s)
\end{itemize}
与乘法器类似，除法器也是分为两类，尽管输入的待运算比特都带有符号位，但接口分为带符号运算和仅限正数两类。
k为辅助比特，t或s为限制QWhile循环次数的经典比特。

此外，除法器有除不尽的问题，因此可以接口函数有如上四种，对应的输入和输出参数分别有如下性质：
\begin{itemize}
	\item QDivider返还余数和商（分别存储在a和c中）时，c.size()=a.size()，但k.size()=a*size()*2+2；
	\item QDivider返还精度和商（分别存储在f和c中）时，c.size()=a.size()，但k.size()=3*size()*2+5；
	\item QDiv返还余数和商（分别存储在a和c中）时，c.size()=a.size()，但k.size()=a*size()*2+4；
	\item QDivider返还精度和商（分别存储在f和c中）时，c.size()=a.size()，但k.size()=a*size()*3+7。
\end{itemize}
如果参数不能满足量子四则运算所需的比特数目，那么计算依然会进行但结果会溢出。
除法的输出比特是c，带精度的除法中a,b,k都不会变，否则b,k不变但a中存储余数。 

结合以上的基础运算接口，测试运算$(4/1+1-3) * 5=10$，具体测试代码如下：
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=量子四则运算测试用例,
label=code:arithemetic
]{code/2.2/arithemetic.py}

\begin{exercise}
	利用以上基础运算的函数接口，学习如何申请寄存器求解$([5/2]+1-4) * 2$，其中$[\cdot]$表示取整。
\end{exercise}




\subsection{量子傅里叶变换}\label{sub:2.2.2}

量子傅里叶变换是离散傅里叶变换的量子实现方案。
已知离散傅里叶变换（DFT）具有如下形式：
\begin{equation}y_k\mapsto\dfrac{1}{\sqrt{N}}\sum\limits_{j=0}^{N-1}x_je^{2\pi ijk/N}\end{equation}
经过简单替换可以直接得到量子傅里叶变换（QFT）
\begin{equation}|x\rangle\mapsto\dfrac{1}{\sqrt{N}}\sum\limits_{k=0}^{N-1}|k\rangle e^{2\pi ixk/N}.\end{equation}
其中$N=2^n$，$n$为量子比特数，且基$|0\rangle,\cdots,|2^n-1\rangle$是$n$量子比特的计算基。并且容易发现，单个量子比特的量子傅里叶变换等价于作用一个H门。

量子傅里叶变换的实质是将空间span$\{|x\rangle\}$中的某个向量$\sum\limits_x\alpha_x|x\rangle$通过变换表示为另一个等价空间span$\{|k\rangle\}$中基向量的线性组合$\sum\limits_k\beta_k|k\rangle$，这一过程可以看作是希尔伯特空间（Hilbert space）上的线性变换，并且这一变换是酉的。

下面首先给出2个量子比特的QFT过程，不妨设其初始态为$|11 \rangle $，并且知道两个量子比特构成的空间其基矢包含$\{|00 \rangle|01 \rangle|10 \rangle|11 \rangle\}$，那么按照上面的变换定义可以得到（11可以认为是二进制中的数字3）：
\begin{equation}
	\begin{split}
		\ket{11}=\ket{3} &\mapsto \frac{1}{2}(e^{\frac{3\pi i 0}{2}}\ket{0}+e^{\frac{3\pi i 1}{2}}\ket{1}+e^{\frac{3\pi i 2}{2}}\ket{2}+e^{\frac{3\pi i 3}{2}}\ket{3})\\
		&=\frac{1}{2}(\ket{0}-i\ket{1}-\ket{2}+i\ket{3})
	\end{split}
\end{equation}

这一变换可以采用如下的量子线路实现：
\begin{figure}[H]
	\centering
\[\Qcircuit @C=1em @R=1em @!R{
	\lstick{\ket{1}}& \gate{H} &\gate{R_2}  &  \qw&\qw \\
	\lstick{\ket{1}}& \qw & \ctrl{-1}    &  \gate{H}&\qw\\
}\]
\end{figure}
其中${\rm R}_2$为旋转门
$$\Qcircuit @C=1.em @R=1.6em {
	 &\gate{\text{R}_2} &\qw }=
\begin{bmatrix} 1 & 0 \\0 
	& e^{2\pi i/2^2} \end{bmatrix}.$$

将该量子线路采用pyqpanda实现：
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=\text{2个量子比特QFT},
label=code:QPanda_qft2
]{code/2.2/QFT_2.py}

可以看到，上面的量子线路比起单个量子比特的QFT多了一个受控旋转门。类似地，量子傅里叶变换在增加量子比特时逐步增加2个、3个、$\cdots$、$n$个受控旋转门，这类似于一个迭代的过程。

更一般的推导：我们把状态$j$写成二进制形式$j=j_{1}j_{2}\cdots j_{n}$，或者更正式地，$j=j_{1}2^{n-1}+j_{2}2^{n-2}+\cdots+j_{n}2^{0}$. 同时，用记号$0.j_{\ell}j_{\ell+1}\cdots j_{m}$表示二进制分数$j_{\ell}/2+j_{\ell+1}/2^2+\cdots+j_{m}/2^{m-\ell+1}$. 则$j/2^{\ell}=j_{1}j_{2}\cdots j_{n-\ell}.j_{n-\ell+1}\cdots j_{n}$。采用这种记号，通过简单的推导可以得到QFT的两种基本表现形式——加法形式与乘法形式：
\begin{equation}\label{eq:qft}
	\begin{split}
		|j\rangle =|j_{1},j_{2},\cdots,j_{n}\rangle &\mapsto
		\dfrac{1}{2^{n/2}}\sum\limits_{k=0}^{2^n-1}e^{2\pi ijk/2^n}|k\rangle\\
		=&\dfrac{1}{2^{n/2}}(|0\rangle+e^{2\pi i0.j_n}|1\rangle)(|0\rangle+e^{2\pi i0.j_{n-1}j_{n}}|1\rangle)\cdots(|0\rangle+e^{2\pi i0.j_{1}j_{2}\cdots j_{n}}|1\rangle)
	\end{split}
\end{equation}
若令
\begin{equation}\phi_{\ell}(j)=\frac{1}{\sqrt{2}}(|0\rangle+e^{2\pi ij2^{-\ell}}|1\rangle)\end{equation}
从而等式\eqref{eq:qft}可表示为
\begin{equation}\label{eq:qft2}
		|j\rangle = |j_{1},j_{2},\cdots,j_{n}\rangle \mapsto
		 \phi_{n}(j)\otimes\phi_{n-1}(j)\otimes\cdots\phi_{1}(j)
\end{equation}

显然，QFT将存在于基向量中的$j$转移到了振幅$e^{2\pi ij2^{-\ell}}$的指数中。 借助QFT及其逆变换，可以实现数据在基向量和振幅之间的相互转化，正是这种特性使得QFT能够在众多叠加态中高效地提取到周期信息。


参考上面的迭代规律，可以给出$n$个量子比特的QFT的量子线路，如图~\ref{fig:QFT}~。值得注意的一点是，当$|j_{1},j_{2},\cdots,j_{n}\rangle = |000\cdots 0\rangle$时，该变换等价于一系列H门分别作用到每个量子比特上。
\begin{figure}[H]
	\centering
	\[
	\Qcircuit @C=1.em @R=1.6em {
		&\lstick{|j_1\rangle} &\gate{\text{H}} &\gate{\text{R}_2} &\gate{\text{R}_3} & \qw &\gate{\text{R}_n} &\qw &\qw &\qw&\cdots& &\qw &\qw &\qw &\qw &\rstick{\phi_{n}(j)}\\
		&\lstick{|j_2\rangle} &\qw &\ctrl{-1} &\qw &\qw &\qw &\gate{\text{H}} &\gate{\text{R}_2} &\qw&\cdots& &\qw &\qw &\qw &\qw &\rstick{\phi_{n-1}(j)} \\
		&\lstick{|j_3\rangle} &\qw &\qw &\ctrl{-2} &\qw &\qw &\qw &\ctrl{-1} &\qw&\cdots& &\qw &\qw &\qw &\qw &\rstick{\phi_{n-2}(j)} \\
		&  &  &  & &  &  &  &  &  &\vdots  &  &  & &\vdots & \\
		&\lstick{|j_{n-1}\rangle} &\qw &\qw &\qw &\ctrl{-4} &\qw &\qw &\qw &\qw&\cdots& &\gate{\text{H}} &\gate{\text{R}_2} &\qw &\qw &\rstick{\phi_{n-3}(j)} \\
		&\lstick{|j_n\rangle} &\qw &\qw &\qw &\qw &\ctrl{-5} &\qw &\qw &\qw&\cdots& &\qw &\ctrl{-1} &\gate{\text{H}} &\qw &\rstick{\phi_{1}(j)} 
	}
	\]
	\caption{QFT}
	\label{fig:QFT}
\end{figure}
其中${\rm CR}_k$为受控旋转门为
$$\Qcircuit @C=1.em @R=1.6em {
	&\qw &\ctrl{1} &\qw&\\
	&\qw &\gate{\text{R}_k} &\qw }=
\begin{bmatrix} 1 & 0&0&0 \\ 0&1&0&0\\0&0&1&0\\0&0&0 
	& e^{2\pi i/2^k} \end{bmatrix}.$$
受控旋转门根据两个量子位之间的纠缠态来执行相位旋转。
从而根据图中的线路，我们可以计算任意量子比特$j_{\ell}$的状态演变，首先通过Hadamard门
\begin{equation}{\rm H}|j_{\ell}\rangle=\dfrac{1}{\sqrt{2}}(|0\rangle+e^{\pi ij_{\ell}}|1\rangle)=\dfrac{1}{\sqrt{2}}(|0\rangle+e^{2\pi i 0.j_{\ell}}|1\rangle) \end{equation}
再依次通过受控量子比特分别是$j_{\ell+k-1}$的${\rm R}_k$门，其中$2\leq k\leq n$. 满足关系
\begin{equation}\label{eq:qft1}
		\text{R}_{k}(|j_{\ell+k-1}\rangle H|j_{\ell}\rangle=
		=|j_{\ell+k-1}\rangle \left(\dfrac{1}{\sqrt{2}}(|0\rangle+e^{\frac{2\pi i j_{\ell+k-1}}{2^{k}}}e^{\frac{2\pi ij_{\ell}}{2}}|1\rangle\right)
\end{equation}

根据公式\eqref{eq:qft1}，计算图中任意量子比特$j_{\ell}$的最终状态是容易的.下面给出$j_{1}$态的线路演变过程，其他态类似的计算过程。
\begin{align*}
	|j_1\rangle \longrightarrow  & \dfrac{1}{\sqrt{2}}(|0\rangle+e^{2\pi i 0.j_{1}}|1\rangle)&\text{Hadamard 变换}\\
	\longrightarrow & \dfrac{1}{\sqrt{2}}(|0\rangle+e^{2\pi i 0.j_{1}j_{2}}|1\rangle ) &\text{受控比特在$|j_{2}\rangle$的旋转门$R_{2}$}\\
	\longrightarrow & \dfrac{1}{\sqrt{2}}(|0\rangle+e^{2\pi i 0.j_{1}j_{2}j_{3}}|1\rangle )&\text{受控比特在$|j_{3}\rangle$的旋转门$R_{3}$}\\
	&~~~\vdots~& \vdots\\
	\longrightarrow & \dfrac{1}{\sqrt{2}}(|0\rangle+e^{2\pi i 0.j_{1}j_{2}\cdots j_{n}}|1\rangle )&\text{受控比特在$|j_{n}\rangle$的旋转门$R_{n}$}\\
	& =\phi_{n}(j)
\end{align*}
从而，上述量子线路的最终输出状态为
\begin{equation}|j_1,j_2,\cdots,j_n\rangle\mapsto\dfrac{1}{\sqrt{2^n}}\bigotimes\limits_{\ell=1}^n (|0\rangle+e^{2\pi i0.j_{\ell}j_{\ell+1}\cdots j_n}|1\rangle)=\phi_{n}(j)\otimes\phi_{n-1}(j)\otimes\cdots\phi_{1}(j)\end{equation}
这与公式\eqref{eq:qft2}是一致的（经过简单换序），即对量子态$|j\rangle$作了QFT。因此，任意量子比特数的QFT能够被下面的pyqpanda量子线路实现:
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=\text{QFT一般形式},
label=code:QPanda_qftn
]{code/2.2/QFT_n.py}

 利用傅立叶变换可以构造加法器，可以构造量子相位估计(QPE)等基本组件，从而可以进一步实现HHL算法或Shor算法等。因此量子傅里叶变换在量子计算中是十分重要的，为此，在Qpanda以及pyqpanda中已经将上面的QFT线路进行了封装，量子傅里叶变换及其逆变换的调用方式如下：

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=\text{QFT及其逆的调用},
label=code:QPanda_iqft
]{code/2.2/qft.py}

\begin{exercise}
	下面请尝试使用pyqpanda构造一个三量子比特的量子傅里叶逆变换的量子线路（可以使用pyqpanda中的QFT接口配合验证）。
\end{exercise}
\begin{exercise}
	已知量子傅里叶变换可以看作是一个线性变换，尝试给出3个量子比特进行QFT所需的变换矩阵（$8\times 8$）。
\end{exercise}

QFT的应用非常广泛，可以将基向量和振幅相互转化，是目前很多主流量子算法的基本组件：
\begin{enumerate}
	\item 利用QFT可以实现QPE求解相位的近似估计，进而可以构造HHL算法求解线性方程组；
	\item 利用QFT可以实现Shor算法求解隐藏子群问题，针对整数分解或者离散对数等困难问题可以实现指数级的加速；
	\item 利用QFT的张量积分解形式，可以实现基于常数的加法器和模运算器，相比其他量子运算器可以节省量子比特数。
\end{enumerate}
针对这三大应用，本书均会介绍，下面先介绍基于QFT如何构造常数算术运算。

\subsubsection{基于QFT的常数算术运算}\label{subsubsec:changshuarit}

\textbf{基于QFT的常数加法器}

利用量子傅里叶变换可以实现常数量子加法器，具体实现思路是利用量子傅里叶变换的张量积分解，将加法运算转化为傅里叶变换的相位求和。参考文献\cite{beauregard2002circuit,takahashi2009quantum}，这里给出基于QFT加法器的具体实现$|x\rangle \rightarrow |x+a\rangle$，其中$a$为常数。通过经典预处理得到$a$做傅里叶展开的相位数组：若将$a$作傅里叶展开，可以得到
\begin{equation} 
	\begin{split}
		|a_{n-1},a_{n-2},\cdots,a_{0}\rangle &=|a\rangle\mapsto\\
		&\dfrac{1}{2^{n/2}}\sum\limits_{k=0}^{2^n-1}e^{2\pi iak/2^n}|k\rangle = \dfrac{1}{2^{n/2}}\bigotimes_{\ell=1}^{n}[|0\rangle+e^{2\pi ia2^{-\ell}}|1\rangle]\\
		=&\dfrac{1}{2^{n/2}}(|0\rangle+e^{2\pi i0.a_{0}}|1\rangle)(|0\rangle+e^{2\pi i0.a_{1}a_{0}}|1\rangle)\cdots(|0\rangle+e^{2\pi i0.a_{n-1}a_{n-2}\cdots a_{0}}|1\rangle).
	\end{split} 
\end{equation}
其中$ 0.a_{\ell}a_{\ell-1}\cdots a_{l-m+1}$表示二进制分数$ a_{\ell}/2+a_{\ell-1}/2^2+\cdots+a_{\ell-m+1}/2^{\ell-m+1} $。
令$ \phi_{\ell}(x)=\frac{1}{\sqrt{2}}(|0\rangle+e^{2\pi ia2^{-\ell-1}}|1\rangle) $，从而等式可表示为
\begin{equation} 
	\begin{split}
		|a_{n-1},a_{n-2},\cdots,a_{0}\rangle=|a\rangle\mapsto&\dfrac{1}{2^{n/2}}\sum\limits_{k=0}^{2^n-1}e^{2\pi iak/2^n}|k\rangle\\
		=& \phi_{n-1}(a)\otimes\phi_{n-2}(a)\otimes\cdots\phi_{0}(a).
	\end{split}
\end{equation}
进而，可以预先得到$a$作傅里叶展开的相位数组$[\theta_{k}(a)]_{k}, k\in[0,n-1]$，其中
\begin{equation}\label{eq:angles}	
	\theta_{k}(a)=2\pi\sum_{j=0}^{k}\frac{a_{j}}{2^{k+1-j}}=2\pi\left(\frac{a_{k}}{2}+\frac{a_{k-1}}{2^2}+\cdots+\frac{a_{0}}{2^{k+1}}\right) ,~~~a_{k}\in\{0,1\}. 
\end{equation}

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=通过经典处理得到相位数组,
label=code:QPanda_getangles
]{code/2.2/getangles.py}

相应地，将$x$作为量子态$|x\rangle$做量子傅里叶变换，可以构造出$n+1$个量子比特数的常数量子加法器，其中$n=\max\{\lceil\log_{2}x\rceil,\lceil\log_{2}a\rceil\}$。具体线路图见下图\ref{fig:conadd}，其中线路图中的RZ门表示为
$\left(\begin{array}{cc}1 & 0 \\0 & e^{i\theta_{k}(a)} \end{array} \right)$。

\begin{figure}[H]
	\centering
	\[
	\Qcircuit @C=1.em @R=1.6em {
		&\lstick{|x_{0}\rangle}  & \multigate{4}{\text{QFT}} & \qw & \qw{/}^{\phi_{0}(x)} &\qw & \gate{Rz(\theta_{0}(a))} &\qw & \qw{/}^{\phi_{0}(x+a)} & \qw & \multigate{4}{\text{QFT$^{\dagger}$}}  & \rstick{|x+a\rangle_{0}}\qw  \\
		&\lstick{|x_{1}\rangle}  & \ghost{\text{QFT}}  & \qw & \qw{/}^{\phi_{1}(x)} &\qw & \gate{Rz(\theta_{1}(a))} &\qw & \qw{/}^{\phi_{1}(x+a)} & \qw & \ghost{\text{QFT$^{\dagger}$}} & \rstick{|x+a\rangle_{1}}\qw   \\
		&&&& &\vdots  &  &  & &\vdots &  & & & & &   \\
		&\lstick{|x_{n-2}\rangle}& \ghost{\text{QFT}} & \qw & \qw{/}^{\phi_{n-2}(x)} &\qw & \gate{Rz(\theta_{n-2}(a))} &\qw& \qw{/}^{\phi_{n-2}(x+a)} & \qw & \ghost{\text{QFT$^{\dagger}$}} & \rstick{|x+a\rangle_{n-2}}\qw \\
		&\lstick{|x_{n-1}\rangle}  & \ghost{\text{QFT}} & \qw & \qw{/}^{\phi_{n-1}(x)} &\qw & \gate{Rz(\theta_{n-1}(a))} &\qw& \qw{/}^{\phi_{n-1}(x+a)} & \qw & \ghost{\text{QFT$^{\dagger}$}} & \rstick{|x+a\rangle_{n-1}}\qw 
	}\]
	\caption{基于QFT的常数加法器(简记为：$+/-$常数)}
	\label{fig:conadd}
\end{figure}


具体实现代码见\ref{code:QFTConAdd}。相应地调用PyQPanda中QFTConAdd函数接口，可以实现$|x+a\rangle$和$|x-a\rangle$的运算。注意到，对于减法利用QFTConAdd.dagger()接口，若$a\le x$，得到结果为$|x-a\rangle$；若$a>x$，得到结果为$|2^{n}-x+a\rangle$。

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=基本QFT的加法线路实现代码,
label=code:QFTConAdd
]{code/2.2/qftconadd.py}

\begin{exercise}
	比较基于UMA的和基于QFT的加法器，可以从量子比特数和线路深度角度分析。
\end{exercise}

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=基于QFT的加法用例测试,
label=code:QPanda_QFTConAdd
]{code/2.2/textQFTConAdd.py}

基于以上QFT常数加法器，相应可以构造出常数模加法器、常数模加乘运算器、常数模乘法器和常数模幂运算器,下面将一一介绍。下面统一符号：模数为$ N\in\mathbb{N}$且其比特长数$n= \lceil \log_{2}N \rceil$，令$ a\in [0,N-1] $为常数。

\textbf{基于QFT的常数模加法器}

若对于变量$x\in[0,N-1]$计算常数模加$a+x \bmod N $，其量子线路实现的主要过程如下：
\begin{description}
	\item[1] 借助辅助比特aux，利用QFT常数加法器计算$x+a-N $。
	\item[2] 通过获得$|x+a-N\rangle$的最高进位比特(aux)是0还是1，判断$x+a-N $是小于0还是大于0。
	\item[3] 若aux=1，即表示$ x+b<N $，则对寄存器$ |x\rangle $执行加$N$操作；若aux=0，即表示 $ x+b\ge N $，不执行操作，进入下一步。
	\item[4] 当前量子寄存器$ |x\rangle $已转化为$ |(x+a)\bmod N\rangle $。为了保证辅助比特不改变状态，通过减$a$和加$a$操作以及通过比较 $(x+a)\bmod N-a $的大小，通过CNOT门操作可以将辅助比特重置为0。
\end{description}
具体线路图如图\ref{fig:conmodadd}所示和相应的实现代码如 所示。
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=常数模加量子线路实现代码,
label=code:ConModAdd
]{code/2.2/conmodadd.py}

下面，给出简单的测试代码$9+7\bmod 11$，测试PyQPanda测试代码如下：

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=常数模加的计算示例,
label=code:QPanda_ConModAdd
]{code/2.2/textConModAdd.py}

\begin{figure}[htbp]
	\centering
	\[
	\Qcircuit @C=1.em @R=1.4em {
		&\lstick{|x\rangle} & \qw{/}^{n} & \multigate{1}{+a} & \multigate{1}{-N}  & \gate{+N} & \multigate{1}{-a} &\qw & \gate{+a} & \rstick{|x+a\bmod N\rangle}\qw  \\
		&\lstick{|0\rangle} & \qw{/}^{1} & \ghost{+a}   &  \ghost{-N} & \ctrl{-1} &\ghost{-a} &\targ & \qw & \rstick{|0\rangle}\qw\gategroup{1}{7}{2}{9}{.7em}{--}
	}\]
	\caption{常数模加运算量子线路(简记为：ADDN)}
	\label{fig:conmodadd}
\end{figure}

\begin{exercise}
	图\ref{fig:conmodadd}中虚线部分表示比较器，其主要目的是为了将辅助比特置零。考虑设计不同的比较器满足一样的计算效果（可以通过增加一个辅助比特来设计）。
\end{exercise}

\textbf{基于QFT的常数模乘法器}

若对于变量$ x,y\in[0,N-1]$计算常数模加乘$ y+ax\bmod N $。首先利用等式：
\begin{equation}
	ax\bmod N=(\ldots((2^{0}ax_0)\bmod N+2^{1}ax_{1})\bmod N+\ldots+2^{n-1}ax_{n-1})\bmod N,
\end{equation}
其中$x=2^0 x_0+2^1 x_1+2^2 x_2+\cdots +2^{n-1}x_{n-1}, x_i\in \{0,1\}$。
由上式可知，实现常数模乘需要$n-1$次常数模加。从而，结合常数模加线路可以实现常数模加乘线路
$|x\rangle|b\rangle\rightarrow|x\rangle|(b+ax)\bmod N\rangle $，具体线路图见\ref{fig:conmodaddmul}所示。

\begin{figure}[H]
	\centering
	\resizebox{.65\linewidth}{!}{
		$$
	   \Qcircuit @C=1em @R=1em @!R{
		\lstick{\ket{x_0}} & \ctrl{5} &   \qw &   \qw    &   \qw & \qw& \qw&   \qw & \qw& \qw&\rstick{\ket{x_0}}\qw\\
		\lstick{\ket{x_1}} &  \qw &  \qw      &\ctrl{4}&  \qw & \qw& \qw&   \qw & \qw& \qw&\rstick{\ket{x_1}}\qw\\
		\vdots&&&&&& &&&&&&&&&&&&&&\lstick{\ket{x}} &\multigate{3}{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a)$ \rotatebox{90}{N}}}&\rstick{\ket{x}}\qw\\
		\lstick{\ket{x_{n-1}}} & \qw &  \qw& \qw& \qw  & \qw      &\qw  &\qw  &\ctrl{2}& \qw&\rstick{\ket{x_{n-1}}}\qw&&&&&&&&&  \\
		&&&&&&&&&&&&&&&\ \triangleq&\\
		\lstick{\ket{b_0}} & \multigate{3}{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^0a)$ \rotatebox{90}{N}}} &\qw & \multigate{3}{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^1a)$ \rotatebox{90}{N}}}& \qw&\cdot&&\qw& \multigate{3}{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^na)$ \rotatebox{90}{N}}}&\rstick{\ket{b+ax\bmod\ N}_{0}}\qw&&&&&&&&&&&\lstick{\ket{b}}&\ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a)$ \rotatebox{90}{N}}}&\rstick{\ket{b+ax\bmod \ N}}\qw\\
		\lstick{\ket{b_1}} & \ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^0a)$ \rotatebox{90}{N}}}& \qw& \ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^1a)$ \rotatebox{90}{N}}}& \qw&\cdot&&\qw& \ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^na)$ \rotatebox{90}{N}}}&\rstick{\ket{b+ax\bmod\ N}_{1}}\qw\\
		\vdots&&&&&&&&&&&&&&&&&&&&&&\\
		\lstick{\ket{b_{n-1}}} & \ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^0a)$ \rotatebox{90}{N}}} & \qw& \ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^1a)$ \rotatebox{90}{N}}} & \qw&\cdot&&\qw& \ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{D}\ \rotatebox{90}{D}\ $(2^na)$ \rotatebox{90}{N}}}&\rstick{\ket{b+ax\bmod\ N}_{n-1}}\qw\\
	}$$}
	\caption{基于QFT的常数模加乘运算器(简记为：AMULN)}
	\label{fig:conmodaddmul}
\end{figure}

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=常数模加乘量子线路测试用例,
label=code:QPanda_ConModaddmul
]{code/2.2/ConModaddmul.py}


进一步地，为了实现可逆的常数模乘量子线路，根据关系式$ |x\rangle|0\rangle\rightarrow|x\rangle|ax\bmod N\rangle\rightarrow |ax\bmod N\rangle|x\rangle\rightarrow |ax\bmod N\rangle|x-a^{-1}ax\bmod N\rangle=|ax\bmod N\rangle|0\rangle$，即可实现常数模乘量子线路，具体见图\ref{fig:conmodmul},共需要$2n+1$个量子比特。


\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=常数模乘量子线路测试用例,
label=code:QPanda_ConModMul
]{code/2.2/ConModMul.py}


\begin{figure}[ht]
	\centering
	\[\Qcircuit @C=1em @R=1em @!R{
		\lstick{\ket{x}} & \multigate{4}{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a)$ \rotatebox{90}{N}}}& \qw& \multigate{4}{\centering \rotatebox{270}{SWAP}}&\qw& \multigate{4}{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{-1})$ \rotatebox{90}{N}}}&\rstick{\ket{ax\bmod N}}\qw &&&&&&&&&\lstick{\ket{x}} & \multigate{4}{\rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(ax)$ \rotatebox{90}{N}}}& \qw&\rstick{\ket{ax\bmod N}}\qw\\
		&&&&&&&&&&&&&&&&&&&&&&\\
		&&&&&&&&&&&\ \triangleq&&&&\\
		&&&&&&&&&&&&&&&&&&&&&&\\
		\lstick{\ket{0}} & \ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a)$ \rotatebox{90}{N}}}& \qw& \ghost{\rotatebox{270}{SWAP}} &\qw& \ghost{\rotatebox{270}{\rotatebox{90}{A}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{-1})$ \rotatebox{90}{N}}}&\rstick{\ket{0}}\qw &&&&&&&&&\lstick{\ket{0}} & \ghost{\rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a)$ \rotatebox{90}{N}}}& \qw&\rstick{\ket{0}}\qw
	}\]
	\caption{基于QFT的常数模乘运算器(简记为$\text{ConMULTN}$)}
	\label{fig:conmodmul}
\end{figure}

\begin{exercise}
	结合常数模加法器和上述线路，实现常数模加乘法运算器和常数模乘运算器代码。
\end{exercise}

\textbf{基于QFT的常数模幂运算器}

为了计算模幂$ a^{x}\bmod N $，由公式
\begin{equation}
	\begin{split}
		a^{x} \bmod N &= a^{2^0 x_0+2^1 x_1+2^2 x_2+\cdots +2^{n-1}x_{n-1}}\bmod N\\
		& =((a^{2^0x_0}\bmod N)\cdot (a^{2^1x_1}\bmod N)\cdots (a^{2^{n-1}x_{n-1}}\bmod N))\bmod N
	\end{split}
\end{equation}

从而常数模幂可以通过多次常数模乘运算即可，需要多申请一个量子寄存器迭代模加每次的模乘结果，具体线路图见图\ref{fig:conmodexp}。
具体实现过程中需要三个量子寄存器，共需要$3n+1$个量子比特。结合PyQPanda，可以实现模幂的测试（测例：$2*4\bmod 11$）：

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=常数模幂量子线路测试用例,
label=code:QPanda_ConModExp
]{code/2.2/ConModExp.py}

\begin{figure}[ht]
	\centering
	\[\Qcircuit @C=0.7em @R=0.5em @!R{
		\lstick{\ket{x_0}}&   \qw & \ctrl{5} &   \qw &   \qw    &   \qw & \qw& \qw&   \qw & \qw& \rstick{\ket{x_0}}\qw\\
		\lstick{\ket{x_1}}&   \qw &  \qw &  \qw      &\ctrl{4}&  \qw & \qw& \qw&   \qw & \qw& \rstick{\ket{x_1}}\qw\\
		\vdots&&\\
		\lstick{\ket{x_n}}&   \qw & \qw &  \qw& \qw& \qw  & \qw      &\qw  &\qw  &\ctrl{2}& \rstick{\ket{x_n}}\qw  \\
		&\\ 
		\lstick{\ket{0}_{0}} &  \gate{X}& \multigate{4}{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^0})$ \rotatebox{90}{N}}} & \qw& \multigate{4}{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^1})$ \rotatebox{90}{N}}}& \qw&\cdot&&\qw& \multigate{4}{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^n})$ \rotatebox{90}{N}}}& \rstick{\ket{a^x \bmod N}}\qw\\
		\lstick{\ket{0}_{n-1}} &  \qw& \ghost{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^0})$ \rotatebox{90}{N}}} & \qw& \ghost{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^1})$ \rotatebox{90}{N}}}& \qw&\cdot&&\qw& \ghost{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^n})$ \rotatebox{90}{N}}}& \rstick{\ket{a^x \bmod N}}\qw\\
		&&& && &&&&&\\
		&&& && &&&&&\\
		\lstick{\ket{0}}& \qw{/}^{n} & \ghost{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^0})$ \rotatebox{90}{N}}} & \qw& \ghost{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^1})$ \rotatebox{90}{N}}}& \qw&\cdot&&\qw& \ghost{\centering \rotatebox{270}{\rotatebox{90}{Con}\ \rotatebox{90}{M}\ \rotatebox{90}{U}\ \rotatebox{90}{L}\ \rotatebox{90}{T}\ $(a^{2^n})$ \rotatebox{90}{N}}}& \rstick{\ket{0}_{n}}\qw
	}\]
	\caption{基于QFT的常数模幂运算器}
	\label{fig:conmodexp}
\end{figure}

\begin{exercise}
	结合线路和常数模乘运算器，实现常数模幂运算器代码。
\end{exercise}

\subsubsection{变量模运算基本组件}
本小节重点介绍全量子态参与运算的模运算基本组件，不同于\S\ref{subsubsec:changshuarit}节的常数模运算组件---其中将一部分作为常数作经典处理。 下面主要介绍变量模加、二倍模乘、变量模乘、变量模平方、模逆等基础运算组件。以下，均假设模数为$N\in \mathbb{N}$且$n=\lceil\log_{2}N\rceil$。以下的基本组件有些设计思想和文献\cite{roetteler2017quantum}中的思想相似，但个别有不同。

\textbf{变量模加法运算器}

对于两个量子寄存器$|x\rangle,|y\rangle$以及模数$N$，实现$|x+y \bmod N\rangle$，具体实现步骤如下。设$ x,y\in[0,N-1]$，令$|x\rangle$为第一寄存器，$|y\rangle$为第二寄存器。

\begin{description}
	\item[1] 借助一个辅助比特aux1作为加法进位，利用QPanda中的加法器(python中的接口为QAdder，此操作需要额外一个辅助比特aux0)实现$|x+y\rangle$，所得结果寄存在第一寄存器中。
	\item[2] 对第一寄存器和辅助比特aux1做常数模减得到$|x+y-N\rangle$，利用基于QFT的常数加法器(QFTConAdd)。
	\item[3] 根据辅助比特aux1，对$|x+y-N\rangle$做受控加$N$操作：\\
	1）若aux1=1（即表示$ x+y<N $）, 则对第一寄存器执行加$N$操作；\\
	2）若aux1=0（即表示$ x+y\ge N $），不执行相关操作。\\
	当前第一个寄存器中结果为
	$\begin{cases}
		|x+y\rangle, 0\le x+y <N\\
		|x+y-N\rangle, N\le x+y< 2N
	\end{cases} $。\\
	之后的步骤，主要是对辅助比特aux1的复位，实现变量模加的可逆线路。
	\item[4] 最后，通过构造比较器对辅助比特aux1复位。通过对第一个和第二个寄存器执行带进位的减法操作，通过CNOT门操作可以将辅助比特重置为0，最后再对对第一个和第二个寄存器执行不带进位的加法操作(QAdderIgnoreCarry)即可。
\end{description}


变量模加线路图如图\ref{fig:varmodadd}所示，共需要$2n+2$个量子比特。代码示例如下：

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=变量模加量子线路代码实现与测试用例,
label=code:QPanda_varmodadd
]{code/2.2/varmodadd.py}

\begin{figure}[htbp]
	\centering
	\[
	\Qcircuit @C=1.em @R=1.4em {
		&\lstick{|y\rangle} & \qw{/}^{n} & \multigate{3}{\text{Qadder}} & \qw & \qw & \multigate{3}{\text{Qadder$^{\dagger}$}} &\qw & \multigate{2}{\text{Qadder}} & \rstick{|y\rangle}\qw  \\
		&\lstick{|x\rangle} & \qw{/}^{n} & \ghost{\text{Qadder}}   & \sgate{-N}{1} &  \gate{+N} &\ghost{\text{Qadder$^{\dagger}$}} & \qw & \ghost{\text{Qadder}} & \rstick{|x+y\bmod N\rangle}\qw \\
		&\lstick{|aux0\rangle} & \qw{/}^{1} & \ghost{\text{Qadder}}   & \qw &  \qw &\ghost{\text{Qadder$^{\dagger}$}} &\qw & \ghost{\text{Qadder}} & \rstick{|0 \rangle}\qw \\
		&\lstick{|aux1\rangle} & \qw{/}^{1} & \ghost{\text{Qadder}}   & \sgate{-N}{-1} & \ctrl{-2} &\ghost{\text{Qadder$^{\dagger}$}} &\targ & \qw & \rstick{|0\rangle}\qw\gategroup{1}{7}{4}{9}{.7em}{--}
	}\]
	\caption{变量模加运算量子线路}
	\label{fig:varmodadd}
\end{figure}

\begin{exercise}
	思考变量模加和常数模加运算器的不同，分析他们的可应用场景。
\end{exercise}


\textbf{一种特殊的二倍模乘运算器}

下面给出一种特殊的二倍模乘运算器，考虑模数$N$为奇数情形下的二倍模乘，仅需要简单的SWAP门和常数加法操作，相比较常数模乘运算所需的$2n+1$个量子比特，此种线路仅需要$n+1$个量子比特。具体实现思想如下：设模数$N$为奇数且$ n=\lceil\log_{2}(N)\rceil$，求解变量$ x\in[0,N-1]$，设计量子线路计算$ |2x \bmod N\rangle $。
\begin{description}
	\item[1]  借助辅助比特aux，对$|x\rangle$量子寄存器按位向左移一位。此过程的线路仅需从最高位开始，依次和下一低位作交换即可，具体见线路图\ref{fig:lshift}。
	\item[2] 对量子寄存器$|x\rangle$和辅助比特整体做减$N$（利用QFT常数加法器）操作，得到$|2x-N\rangle$。
	\item[3] 通过辅助比特可以对量子寄存器$|x\rangle$做常数加$N$操作。从而，当前量子寄存器的结果为
	$$ \begin{cases}
		|2x\rangle|1\rangle, 0\le 2x < N\\
		|2x-N\rangle|0\rangle, N\le 2x< 2N
	\end{cases} $$
	\item[4] 最后，通过最低位比特对辅助比特做复位操作：\\
	1）若寄存器中存的结果是$|2x\rangle$，即为偶数，最低位比特为$|0\rangle$。X(LSB($2x$))门之后，此时LSB($2x$)=1且aux的状态为1，对aux做X门操作。进而，aux的状态变为$|0\rangle$。\\
	2）若寄存器中存的结果是$|2x-N\rangle$，由于$N$是奇数，所以$2x-N$为奇数，最低位比特为$|1\rangle$。X(LSB($2x-N$))操作后，此时LSB($2x-N$)=0且aux的状态为$|0\rangle$，对aux不执行X门操作。\\
	最后，对第一寄存器的LSB再做X门操作，完成LSB的复位，从而可逆的量子线路，其结果$|2x\bmod N\rangle$存在第一寄存器中。
\end{description}
对比文献\cite{roetteler2017quantum}中的$n+2$个量子比特数，此变量二倍模乘量子线路仅需要$n+1$个量子比特。

代码示例如下：
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=变量二倍乘的测试用例,
label=code:QPanda_varmoddou
]{code/2.2/varmoddou.py}


\begin{figure}[htbp]
	\centering
	\[
	\Qcircuit @C=1.em @R=1.6em {
		&\lstick{|x_{0}\rangle} & \qw & \qw & \qw  & \qw & \qw  & \qw & \qw  & \qw & \qw &\qw & \qswap &\qw &\qw & \rstick{|0 \rangle}\qw\\
		&\lstick{|x_{1}\rangle} & \qw & \qw & \qw  & \qw & \qw  & \qw & \qw  & \qw & \qswap & \qw & \qswap\qwx & \qw  & \qw & \rstick{|x_{0} \rangle}\qw \\
		&\lstick{|x_{2}\rangle} & \qw & \qw & \qw  & \qw & \qw  & \qw & \qw  & \qw & \qswap\qwx  & \qw  & \qw& \qw  & \qw  & \rstick{|x_{1} \rangle}\qw\\
		& &\vdots  &  &&& &&& & &\vdots &  & & & & &   \\
		&\lstick{|x_{n-2}\rangle} & \qw & \qw &\qw & \qw & \qswap  & \qw & \qw & \qw  & \qw & \qw & \qw  & \qw  & \qw & \rstick{|x_{n-3} \rangle}\qw\\
		&\lstick{|x_{n-1}\rangle} & \qw & \qw & \qswap & \qw & \qswap\qwx  & \qw & \qw & \qw  & \qw & \qw & \qw  & \qw & \qw  & \rstick{|x_{n-2} \rangle}\qw\\
		&\lstick{|0\rangle} & \qw & \qw & \qswap\qwx  & \qw & \qw & \qw & \qw & \qw  & \qw & \qw & \qw  & \qw & \qw & \rstick{|x_{n-1} \rangle}\qw 
	}\]
	\caption{向左移位实现二倍乘操作}
	\label{fig:lshift}
\end{figure}


\begin{figure}[htbp]
	\centering
	\[
	\Qcircuit @C=1.em @R=1.6em {
		&\lstick{|x_{0}\rangle} & \qw &  \multigate{4}{2x} & \qw & \qw  &  \multigate{4}{-N} & \qw  &\multigate{3}{+N}  & \gate{X} & \ctrl{4}  & \gate{X} & \qw & \rstick{|(2x \bmod N)_{0} \rangle}\qw\\
		&\lstick{|x_{1}\rangle} & \qw & \ghost{\text{2x}} & \qw & \qw  & \ghost{-N} & \qw  & \ghost{+N}  &\qw & \qw & \qw & \qw & \rstick{|(2x \bmod N)_{1} \rangle}\qw\\
		& &\vdots  &  &&& &&& & &\vdots &    \\	     
		&\lstick{|x_{n-1}\rangle} & \qw & \ghost{\text{2x}} & \qw & \qw  & \ghost{-N} & \qw & \ghost{+N}  &\qw & \qw & \qw & \qw  & \rstick{|(2x \bmod N)_{n-1} \rangle}\qw\\
		&\lstick{|aux\rangle} & \qw & \ghost{\text{2x}} & \qw & \qw  & \ghost{-N} & \qw   & \ctrl{-1}  &\qw  &\targ & \qw & \qw  & \rstick{|aux \rangle}\qw 
	}\]
	\caption{变量二倍模乘运算器(简记为：MDbl)}
	\label{fig:varmoddou}
\end{figure}

\begin{exercise}
	结合线路图，实现左移二倍乘和二倍模乘代码。思考此二倍模乘法器为什么不适应于非奇数的模数。
\end{exercise}

\textbf{变量模乘法运算器}

结合变量二倍模乘和变量模加量子运算器，可以实现奇模数下的变量模乘运算器。设模数$N$为奇数，针对变量$ x,y\in[0,N-1]$，利用量子线路计算$ |x\cdot y \bmod N\rangle $。其实现基本原理如下：
已知有表达式$ x=\sum_{i=0}^{n-1}x_{i}2^{i} $，计算
\begin{equation}
	\begin{aligned}
		x\cdot y \bmod N &=\sum_{i=0}^{n-1}x_{i}2^{i}\cdot y\bmod N=x_{0}y+2(x_{1}y+2(x_{2}y+\cdots\\
		& +2(x_{n-2}y+2(x_{n-1}y\bmod N)\bmod N)\bmod N)\cdots)\bmod N
	\end{aligned}
\end{equation}
类比经典中的高位到低位的快速模乘运算，所以，可转换为一系列的受控的变量模加线路以及$n-1$次的二倍模乘线路。具体流程图可见图\ref{fig:modmul}。此线路所需比特数为$3n+2$，得到$ |x\rangle|y\rangle|0\rangle \rightarrow |x\rangle|y\rangle|x\cdot y\bmod N\rangle$。具体测试接口如下：

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=变量模乘的测试用例,
label=code:QPanda_varmodmul
]{code/2.2/varmodmul.py}

\begin{figure}[H]
	\centering
	\resizebox{.70\linewidth}{!}{
		$$
		\Qcircuit @C=0.7em @R=1.em {
			&\lstick{|x_{0}\rangle} & \qw  & \qw & \qw & \qw  & \qw  &\cdots & &\qw &\qw    &\ctrl{5}&\qw & \rstick{|x_{0}\rangle}\qw\\
			&\lstick{|x_{1}\rangle} & \qw  & \qw & \qw & \qw  & \qw &\cdots &  &\ctrl{4}  &\qw &\qw &\qw & \rstick{|x_{1}\rangle}\qw\\
			&  &\vdots  &  &&& &&& & &\vdots &      \\	     
			&\lstick{|x_{n-2}\rangle} & \qw & \qw & \qw& \ctrl{2}  & \qw  &\cdots  & &\qw  &\qw &\qw &\qw & \rstick{|x_{n-2}\rangle}\qw\\
			&\lstick{|x_{n-1}\rangle} & \qw &\ctrl{1}  & \qw & \qw & \qw  &\cdots & &\qw &\qw &\qw &\qw& \rstick{|x_{n-1}\rangle}\qw\\
			&\lstick{|y\rangle} & \qw{/}^{n} &  \multigate{2}{\text{MAdd}} & \multigate{2}{\text{MDbl}} &    \multigate{2}{\text{MAdd}} & \multigate{2}{\text{MDbl}} &\cdots & &  \multigate{2}{\text{MAdd}}  & \multigate{2}{\text{MDbl}} &\multigate{2}{\text{MAdd}} &\qw & \rstick{|y\rangle}\qw\\
			&\lstick{|0\rangle} & \qw{/}^{n} & \ghost{\text{MAdd}} &  \ghost{\text{MDbl}}&  \ghost{\text{MAdd}} &  \ghost{\text{MDbl}} & \cdots  & &  \ghost{\text{MAdd}}  &  \ghost{\text{MDbl}} & \ghost{\text{ModAdd}}&\qw & \rstick{|x*y \bmod N\rangle}\qw\\
			&\lstick{|0\rangle} & \qw{/}^{2} & \ghost{\text{MAdd}} &  \ghost{\text{MDbl}}&  \ghost{\text{MAdd}} &  \ghost{\text{MDbl}} & \cdots  & &  \ghost{\text{MAdd}}  &  \ghost{\text{MDbl}} & \ghost{\text{MAdd}}&\qw & \rstick{|0\rangle}\qw
		}$$}
	\caption{变量模乘运算器}
	\label{fig:modmul}
\end{figure}

\begin{exercise}
	结合二倍模乘和模加线路，实现变量模乘代码。
\end{exercise}

\textbf{变量模平方运算器}

若变量$x\in[0,N-1]$，利用量子线路计算$ |x^{2} \bmod N\rangle$，计算
\begin{equation}
	\begin{aligned}
		x^{2} \bmod N&=\sum_{i=0}^{n-1}x_{i}2^{i}\cdot x\bmod N=x_{0}x+2(x_{1}x+2(x_{2}x+\cdots \\
		&+2(x_{n-2}x+2(x_{n-1}x\bmod N)\bmod N)\bmod N)\cdots)\bmod N
	\end{aligned} 
\end{equation}

类比经典中的高位到低位的快速模乘运算，可转换为一系列受控的变量模加线路以及$n-1$次的变量二倍乘线路。具体流程图可见图\ref{fig:modsqr}。此线路所需比特数为$2n+2$，得到$ |x\rangle|0\rangle\rightarrow |x\rangle|x^{2}\bmod N\rangle$。变量平方模相比较变量模乘节省一个$n$比特量子寄存器，仅需要多一个辅助比特将$x_{i} $的受控信息转移到辅助比特上，之后根据辅助比特的受控性做变量模加即可，具体实现代码如\ref{code:varmodsqr}。利用PyQPanda的测试接口如下（测试$7^2\bmod 11$）：

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=变量模平方的实现代码,
label=code:varmodsqr
]{code/2.2/modsqr.py}

\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1}\scriptsize\ttfamily,
caption=变量模平方的测试用例,
label=code:QPanda_varmodsqr
]{code/2.2/varmodsqr.py}


\begin{figure}[H]
	\centering
	\resizebox{.70\linewidth}{!}{
		$$
		\Qcircuit @C=0.5em @R=0.9em {
			&\lstick{|0\rangle} & \qw  & \targ & \ctrl{1}  &\targ &\targ & \ctrl{1} & \targ &\qw &\cdots &  &\targ & \targ &\ctrl{1} &\targ & \rstick{|0\rangle}\qw\\
			&\lstick{|x_{0}\rangle} & \qw  & \qw & \multigate{6}{\text{MAdd}}&\qw &\qw & \multigate{6}{\text{MAdd}} \ &\qw &\qw &\cdots &  &\qw &\ctrl{-1} &\multigate{6}{\text{MAdd}} &\ctrl{-1} & \rstick{|x_{0}\rangle}\qw \\
			&\lstick{|x_{1}\rangle} & \qw  & \qw  & \ghost{\text{MAdd}} &\qw &\qw &  \ghost{\text{MAdd}} &\qw&\qw &\cdots &  &\ctrl{-2} &\qw &\ghost{\text{MAdd}} &\qw & \rstick{|x_{1}\rangle}\qw \\
			&  &\vdots  &  &&& && &\vdots &  & \\	 
			&\lstick{|x_{n-2}\rangle} & \qw  & \qw & \ghost{\text{MAdd}}&\qw  &\ctrl{-4}  &  \ghost{\text{MAdd}} &\qw &\qw &\cdots &  &\qw &\qw  &\ghost{\text{MAdd}} &\qw & \rstick{|x_{n-2}\rangle}\qw\\
			&\lstick{|x_{n-1}\rangle} & \qw  & \ctrl{-5} & \ghost{\text{MAdd}} & \ctrl{-5} &\qw &  \ghost{\text{MAdd}} & \ctrl{-5} &\qw &\cdots &  &\qw &\qw  &\ghost{\text{MAdd}} &\qw & \rstick{|x_{n-1}\rangle}\qw\\
			&\lstick{|0\rangle} & \qw{/}^{n} & \qw  & \ghost{\text{MAdd}} & \multigate{1}{\text{MDbl}}  &\qw &  \ghost{\text{MAdd}}  & \multigate{1}{\text{MDbl}} &\qw &\cdots &   & \multigate{1}{\text{MDbl}} &\qw  &\ghost{\text{MAdd}} &\qw & \rstick{|x^2\bmod N\rangle}\qw\\
			&\lstick{|0\rangle} & \qw{/}^{2} &\qw  & \ghost{\text{MAdd}} &  \ghost{\text{MDbl}} &\qw &  \ghost{\text{MAdd}}  &  \ghost{\text{MDbl}} &\qw &\cdots &  &  \ghost{\text{MDbl}} &\qw &\ghost{\text{MAdd}} &\qw & \rstick{|0\rangle}\qw		
		}$$}
	\caption{变量模平方运算器}
	\label{fig:modsqr}
\end{figure}

\begin{exercise}
	利用以上量子模运算基础组件，设计量子运算器求解$2*(4+3^3)\bmod 11$，保证以最少的量子比特数实现上述运算。
\end{exercise}



\subsection{量子相位估计}\label{sub:2.2.3}


量子相位估计(QPE)是量子计算中最重要的子程序之一。它是许多量子算法的核心模块。QPE可以求解${\rm U}|\psi\rangle=e^{2\pi i\theta}|\psi\rangle$中的$\theta$，其中$\psi$为幺正算子${\rm U}\in\mathbb{C}^{2^m\times2^m}$的特征向量，$e^{2 \pi i\theta}$ 是相应的特征值。由于 $U$ 是酉的，因此其所有特征值的范数均为 1 。$\theta$是相位信息，所以满足$\theta\in [0,1)$。

利用QPE算法可以求解
\begin{equation}{\rm QPE}({\rm U},|0\rangle_n|\psi\rangle_m)=|\Tilde{\theta}\rangle_n|\psi\rangle_m.\end{equation}
从而，求得的$\Tilde{\theta}$为$2^n\theta$的$n$比特近似。下面将结合小示例开始介绍QPE的具体实现思想。

\begin{example}\label{exam:2.2.2}
	选取一个我们较熟悉的$U1$门，并使用量子相位估计来估计它的相位。已知：
	\begin{equation}
		U1(\frac{\pi}{4})|1\rangle=\left[\begin{array}{cc}
			1 & 0 \\
			0 & e^{\frac{i\pi}{4}}
		\end{array}\right]\left[\begin{array}{l}
			0 \\
			1
		\end{array}\right]=e^{\frac{i \pi}{4}}|1\rangle
	\end{equation}
	即$U1(\frac{\pi}{4})|1\rangle=e^{2\pi i\theta}|1\rangle$，我们期望利用\text{QPE}找到$\theta=\frac{1}{8}$。
	在这个例子中，我们将使用三个量子比特并获得一个确切的结果（不是估计！）。
	
	
	首先制备好量子态，准备三个控制比特和一个工作比特，具体实现线路图如图\ref{fig:QPEexam 2.2.1}。随后，设计量子电路，其中工作比特作为酉运算符 $U1$ 的特征向量，我们通过应用 $X$ 门来初始化 $|\psi\rangle=|1\rangle$，对前三个控制比特执行Hadamard门操作，即
	\begin{equation}
		H(|0\rangle_{3})\otimes X(|0\rangle)= \frac{1}{\sqrt{2^3}}(|0\rangle+|1\rangle)^{\otimes 3}\otimes |1\rangle
	\end{equation}
	随后依次对$|\psi\rangle$做受控的$U1^{2^{i}},i=0,1,2$操作，得到：
	\begin{equation}
		\begin{aligned}
			\frac{1}{\sqrt{2^3}}(|0\rangle+|1\rangle)^{\otimes 3}\otimes|1\rangle &\stackrel{CU1^{2^i}}{\longrightarrow} \frac{1}{\sqrt{2^3}}\bigotimes_{i=0}^{3}(|0\rangle+e^{\frac{2^{i}i\pi}{4}}|1\rangle)\otimes|1\rangle \\
			& =  \frac{1}{\sqrt{2^3}}\sum_{i=0}^{7}e^{2\pi i \theta k}|k\rangle\otimes|1\rangle, \theta=\frac{1}{8}.
		\end{aligned}
	\end{equation}
	此时，相位的信息已经存储在三个控制比特的振幅信息中，下面通过对前三个控制比特做量子傅里叶逆变换(IQFT)可以将振幅上的相位信息转移到基向量上。
	\begin{equation}
		\begin{aligned}
			\frac{1}{\sqrt{2^3}}\sum_{k=0}^{7}e^{2\pi i \theta k}|k\rangle &\stackrel{IQFT}{\longrightarrow} \frac{1}{2^3}\sum_{k=0}^{7}e^{2\pi i \theta k}\sum_{j=0}^{7}e^{-\frac{2\pi i j k}{8}}|j\rangle \\
			& =  \frac{1}{2^3}\sum_{k=0}^{7}\sum_{j=0}^{7}e^{-2\pi i k(8\theta-j)/8}|j\rangle.
		\end{aligned}
	\end{equation}
	由于，我们已知$\theta=1/8$，理论上将以1的概率测量得到1，实际测量也是如此，见代码\ref{code:QPanda_qpe1}中的输出结果。
	
	\lstinputlisting[
	style=PythonStyle,
	numbers=left,
	linewidth=0.94\columnwidth,
	xleftmargin=0.06\columnwidth,
	basicstyle=\linespread{1}\scriptsize\ttfamily,
	caption=例\ref{exam:2.2.2}的QPE求解实现代码,
	label=code:QPanda_qpe1
	]{code/2.2/qpe.py}
	
	
	\begin{figure}[H]
		\centering
		\[
		\Qcircuit @C=1.em @R=1.6em {
			&\lstick{|0\rangle} &\gate{\text{H}} &\ctrl{3} &\qw &\qw  &\qw &\multigate{2}{\text{QFT}^{-1}_{n}} &\meter \\
			&\lstick{|0\rangle} &\gate{\text{H}} &\qw &\qw  &\ctrl{2}  &\qw &\ghost{\text{QFT}^{-1}_{n}} &\meter \\
			&\lstick{|0\rangle} &\gate{\text{H}} &\qw &\qw  &\qw &\ctrl{1} &\ghost{\text{QFT}^{-1}_{n}} &\meter \\
			&\lstick{|0\rangle} &\gate{\text{X}} &\gate{\text{U1}^{2^0}} &\qw &\gate{\text{U1}^{2}}  &\gate{\text{U1}^{2^{2}}} &\qw &\qw
		}
		\]
		\caption{针对例子\ref{exam:2.2.2}的QPE实现线路}
		\label{fig:QPEexam 2.2.1}
	\end{figure}
	
\end{example}

结合上述的例子，我们可以知道QPE是在QFT的基础上构造的。注意到，QPE量子算法需要已知构造好的给定算符$U$的特征向量$|\psi\rangle$，从而，QPE主要有如下步骤：
\begin{enumerate}
	\item  制备控制寄存器和工作寄存器，工作寄存器寄存特征向量$|\psi\rangle$的值；
	\item  通过Hadmard门操作将控制寄存器处理成叠加态；
	\item  通过一系列特殊旋转量子门操作将${\rm U}$的特征值信息分解转移到控制量子寄存器的振幅上；
	\item  对辅助量子比特执行傅里叶逆变换，将振幅上的相位信息转移到基向量上；
	\item  对辅助量子比特的基向量分别进行测量后综合可得到特征值的相位信息。
\end{enumerate}

最后，我们给出QPE实现的具体数学原理和算法成功概率。已知两个寄存器组成的$n+m$维量子态$|0\rangle_n|\psi\rangle_m$为${\rm U}$的特征向量。首先对第一个寄存器中$n$个量子比特分别进行Hadamard门操作。

对于任给的量子比特$a|0\rangle+b|1\rangle$，基于幺正算符${\rm U}$定义受控量子门${\rm CU}^{2^t}$，使得
\begin{equation}{\rm CU}^{2t}(a|0\rangle+b|1\rangle)\bigotimes|\psi\rangle=(a|0\rangle+e^{2\pi i\varphi 2^t}b|1\rangle)\bigotimes|\psi\rangle.\end{equation}

借助该量子门可以将相位$\varphi$转移到量子比特$a|0\rangle+e^{2\pi i\varphi2^t}b|1\rangle$的振幅上。经过简单的代数计算，可以得到第一个寄存器的最终状态为
\begin{equation}|\phi\rangle=\dfrac{1}{2^{n/2}}\bigotimes\limits_{t=0}^{n-1}(|0\rangle+e^{2\pi i\varphi2^t}|1\rangle)=\dfrac{1}{2^{n/2}}\sum\limits_{k=0}^{2^n-1}e^{2\pi i\varphi k}|k\rangle.\end{equation}
对$|\phi\rangle$进行量子傅里叶逆变换，可得


\begin{equation}
	\begin{split}
		{\rm QFT}^{-1}|\phi\rangle=&\dfrac{1}{2^{n/2}}\sum\limits_{k=0}^{2^n-1}e^{2\pi i\varphi k}\left(\dfrac{1}{2^{n/2}}\sum\limits_{j=0}^{2^n-1}e^{-\frac{2\pi ikj}{2^n}}|j\rangle\right)\\
		=&\dfrac{1}{2^n}\sum\limits_{k=0}^{2^n-1}\sum\limits_{j=0}^{2^n-1}e^{-\frac{2\pi ik}{2^n}(j-2^n\varphi)}|j\rangle
	\end{split}
\end{equation}
如果存在整数$j_0=2^n\varphi$，则测量第一个寄存器可以以概率1稳定得到量子态$|2^n\varphi\rangle$。否则记$j_0=\left[2^n\varphi\right]$，即
\begin{equation}2^n\delta=\lvert x_0-2^n\varphi\rvert < \frac{1}{2}.\end{equation}
此时测量第一个寄存器得到$|j_0\rangle$的概率为
\begin{equation}
	\begin{split}
		P_{j_0}=&\left(\left\langle  j_{0}\left|\dfrac{1}{2^n}\sum\limits_{k=0}^{2^n-1}\sum\limits_{j=0}^{2^n-1}e^{\frac{-2\pi ik}{2^n}(j-2^n\varphi)}\right|j_{0}\right\rangle\right)^2\\
		=&\left(\left\langle j_{0}\left|\dfrac{1}{2^n}\sum\limits_{k=0}^{2^n-1}e^{-\frac{2\pi ik}{2^n}(j_0-2^n\varphi)}\right|j_{0}\right\rangle\right)^2\\
		=&\dfrac{1}{2^{2n}}\left|\sum\limits_{k=0}^{2^n-1}e^{2\pi ik\delta}\right|^2
		= \dfrac{1}{2^{2n}}\left| \dfrac{2\sin{\pi2^n\delta}}{2\sin{\pi\delta}}\right|^2
		\ge \dfrac{1}{2^{2n}}\left|\dfrac{2^{n+1}\delta}{\pi\delta} \right|^2
		= \dfrac{4}{\pi^2}
	\end{split}
\end{equation}

可知，当$2^n\varphi$不为整数时依然可以以不低于$\dfrac{4}{\pi^2}$的概率测量得到$|j_0\rangle$。 将第一个寄存器测量结果（二进制字符串 $\phi_{1} \phi_{2} \cdots \phi_{n}$）除以 $2^{n}$ 后，即得到相位 $\theta=0.\phi_{1} \phi_{2} \cdots \phi_{n}$。 比如测量结果是$0001(n=4)$，则除以$2^{4}$后，可得到相位为$1/16$。 注意到，辅助比特的个数$n$越大，测量得到的精确度也就越高。


QPE的量子线路如图所示：
\begin{figure}[H]
	\centering
	\[
	\Qcircuit @C=1.em @R=1.6em {
		&\lstick{|0\rangle} &\gate{\text{H}} &\ctrl{4} &\qw&\cdots& &\qw  &\qw &\multigate{3}{\text{QFT}^{-1}_{n}} &\meter \\
		& &\vdots & & & & & &\vdots \\
		&\lstick{|0\rangle} &\gate{\text{H}} &\qw &\qw&\cdots&  &\ctrl{2}  &\qw &\ghost{\text{QFT}^{-1}_{n}} &\meter \\
		&\lstick{|0\rangle} &\gate{\text{H}} &\qw &\qw &\cdots& &\qw &\ctrl{1} &\ghost{\text{QFT}^{-1}_{n}} &\meter \\
		&\lstick{|\psi\rangle} &\qw{/}^{m} &\gate{\text{U}^{2^0}} &\qw&\cdots& &\gate{\text{U}^{2^{n-2}}}  &\gate{\text{U}^{2^{n-1}}} &\qw &\qw
	}
	\]
	\caption{QPE的一般量子线路}
	\label{fig:QPE}
\end{figure}



\begin{exercise}
	考虑使用受控$Y$门进行实验，设计QPE量子线路并尝试得到预期的结果？（提示：记住要确保 $|\psi\rangle$ 是$Y$的特征向量。）
\end{exercise}	




\subsection{Shor算法及其应用}\label{sub:2.2.4}


在前文所述的各种量子计算的辅助工具基础上，Shor算法第一次实现了具有现实意义的量子计算优越性的大门。该算法最早由美国数学家Peter W. Shor在1994年提出\cite{shor1994algorithms}，算法充分利用了量子的叠加态特性与纠缠态特性，在特定问题的求解上对目前最高效的经典数学算法实现了亚指数级别乃至指数级别的加速效果。

Shor算法能够高效求解的这类问题在数学上可以被归纳为——阿贝尔群的隐藏子群问题，要解释这个概念需要理解一些比较抽象、晦涩的术语，但这显然不是本书的目的，所幸这类问题中我们最关心的两个是易于理解的且有现实对应的，这两个问题就是整数分解问题与离散对数问题(Discrete Logarithms Problem, DLP)。

对这两个问题的特殊关心首先是由于其在数学发展中所具有的特殊含义。像整数分解算法的演进几乎伴随了整个数学的发展史，从两千年前的Eratosthenes筛法到20世纪的二次筛法、数域筛法，尽管前人在这一问题上付出了巨大的努力，但是将算法的时间复杂度下降到多项式级别的目标却始终没有达到。此外，关注这两个问题的另一重要原因或许也是多数人关注Shor算法的直接原因就是其在当代密码学中的重要地位。公钥思想的诞生可以看作是密码学由传统走向现代的一个分水岭，RSA算法以及ECC算法作为公钥密码算法中最具代表性的两个密码算法，其各自依赖的数学困难问题恰好就是整数分解问题与离散对数问题。换句话说，如果整数分解问题与离散对数问题能够被高效地求解，即多项式时间复杂度求解，那么，RSA加密算法以及ECC加密算法的安全性将失去根基。

下面重点讲解如何借助Qpanda使用Shor算法完成整数分解与离散对数问题的求解。首先给出Shor算法求解整数分解的量子线路部分，其中$N$是待分解的数字，$n=\lceil \log_{2}N \rceil $，$a$是选取的随机数，要求$\gcd(a,N)=1$

\begin{figure}[H]
	\centering
	\resizebox{.85\linewidth}{!}{
$$\Qcircuit @C=0.6em @R=0.8em {
	&\lstick{|0\rangle} &\gate{\text{H}} &\qw &\qw &\qw&\cdots& &\qw &\qw  &\ctrl{6}  &\multigate{5}{\text{QFT}^{-1}}  &\meter &\cw \\
	&\lstick{|0\rangle} &\gate{\text{H}} &\qw &\qw &\qw&\cdots & &\qw &\ctrl{5} &\qw   &\ghost{\text{QFT}^{-1}}  &\meter &\cw \\ 
	&\lstick{|0\rangle} &\gate{\text{H}} &\qw &\qw &\qw&\cdots& &\ctrl{4} &\qw &\qw  &\ghost{\text{QFT}^{-1}} &\meter &\cw \\
	& &\vdots & & & &\vdots & & & &  \\
	&\lstick{|0\rangle} &\gate{\text{H}} &\qw &\ctrl{2} &\qw&\cdots& &\qw &\qw &\qw  &\ghost{\text{QFT}^{-1}}  &\meter &\cw \\
	&\lstick{|0\rangle} &\gate{\text{H}} &\ctrl{1} &\qw &\qw&\cdots & &\qw &\qw &\qw  &\ghost{\text{QFT}^{-1}}  &\meter &\cw \\ 
	&\lstick{|1\rangle} &\qw{/} &\gate{a \bmod N}  &\gate{a^2 \bmod N} &\qw &\cdots& &\gate{a^{2^{t-3}} \bmod N}  &\gate{a^{2^{t-2}} \bmod N} &\gate{a^{2^{t-1}} \bmod N} &\qw&\qw&\qw
}$$}
\caption{Shor算法量子线路}
\label{fig:shor}
\end{figure}

可以看到，前文介绍的模数运算组件与量子傅里叶变换组件都是Shor算法线路的重要组成部分。

接下来给出Shor算法分解整数的具体流程，首先，通过简单的分析可以得到，分解一个数字$N$，可以通过寻找定数字$a$的周期来实现，即
\begin{equation}
	a^r\equiv 1 \bmod N, \gcd(a,N)=1
\end{equation}
下面的流程将用于寻找周期$r$
\begin{enumerate}
	\item 初始化$t$个量子比特作为第一个寄存器，然后初始化$O(n)$个量子比特作为第二个寄存器，并给第二个比特赋值1，得到量子态
	\begin{equation}
		\varphi = \ket{0}_{t}\otimes\ket{0\cdots 001}
	\end{equation}
	\item 对第一个寄存器作量子傅里叶变换制备叠加态，对于初态$\ket{0}$来说，这一作用等价于对每个量子比特作用一个Hadamard门，得到下面的量子态
	\begin{equation}
		\varphi=\frac{1}{2^{t/2}}\sum_{j=0}^{M-1}\ket{j}\ket{1}
	\end{equation}
    其中令$2^{t}=M$；
	\item 对两个量子寄存器进行如图所示的模指数运算，这部分能够高效计算叠加态，得到
	\begin{equation}\varphi=\frac{1}{2^{t/2}}\sum_{j=0}^{M-1}\ket{j}\ket{a^j \bmod N}
	\end{equation}
	上面的量子态也能够近似地写为
	\begin{equation}\varphi \approx \frac{1}{2^{t/2}\sqrt{r}}\sum_{s=0}^{r-1}\sum_{j=0}^{M-1}e^{2\pi isj/r}\ket{j}\ket{a_{js}}
	\end{equation}
	\item 对上面的第一个量子寄存器进行量子傅里叶逆变换，得到
	\begin{equation}\varphi \approx \frac{1}{\sqrt{r}}\sum_{s=0}^{r-1}\ket{s2^t/r}\ket{a_{js}}\end{equation}
	\item 对第一个量子寄存器进行测量得到$s/r$的估计
\end{enumerate}
得到上面的估计后使用连分数算法就能够得到正确的周期$r$，这个过程中如果得到的周期是奇数，则重新选取$a$，进行下一轮求解，否则通过欧几里得算法能够得到$N$的整数分解。

下面详细说明经典后处理的实现过程---连分数展开\cite{nielsen2002quantum}：
对结果量子态的第一个寄存器进行测量，可以得到$|[\dfrac{2^ts}{r}]\rangle,0\le s\le r$。 其中，
\begin{equation}
 \left|\left[\dfrac{2^ts}{r} \right]-\dfrac{2^ts}{r} \right|\le \dfrac{1}{2}
\end{equation}
即
\begin{equation}
	\left|\dfrac{\left[ 2^ts/r\right]}{2^t}-\dfrac{s}{r} \right|\le\dfrac{1}{2^{t+1}}
\end{equation}

如果$r=2^k,k\in\mathbb{Z},k\le t$，那么$\dfrac{2^ts}{r}$均为整数，对第一个寄存器进行大量测量，得到每个状态的概率$\dfrac{1}{r}$或者总状态数，也能求得整数$r$。
如果取$t=2n+1+\left[\log(2+\dfrac{1}{2\epsilon})\right]$，那么可以得到二进制展开精度$2n+1$位的相位估计结果，且测量得到该结果的概率至少为$\dfrac{1-\epsilon}{r}$。所以， 一般取$t=2n$ \cite{shor1994algorithms}。

上面的内容在理论上给出了Shor算法的流程，接下来通过两个例子帮助理解:

\noindent \textbf{分解$N=35$，Shor算法中的经典流程：}
\begin{itemize}
	\item 选定随机数$a=4$，检验$\gcd(4,35)=1$；
	\item 假设利用量子线路与后处理得到$a$的周期$r=6$，即\begin{equation}4^6\equiv 1\bmod 35\end{equation}
	\item 计算$\gcd(a^{r/2}-1, N) \&\gcd(a^{r/2}+1, N)$，从而有\begin{equation}\gcd(63,35)=7,\gcd(65,35)=5\end{equation}这样就得到了35的整数分解。
\end{itemize}

\noindent \textbf{分解$N=35$，Shor算法中的量子计算流程与后处理：}
\begin{itemize}
	\item 取定$n=\lceil \log_{2}N \rceil = 6$，申请两个量子寄存器$\ket{0}_{12}\ket{1}_{O(n)}$
	\item 对第一个寄存器作用Hadamard门，得到
	\begin{equation}
		\varphi = \frac{1}{64}\sum_{j = 0}^{4095}\ket{j}\ket{1}
	\end{equation}
	\item 对量子寄存器作用模指数运算组件，得到
	\begin{equation}
		\varphi =  \frac{1}{64}\sum_{j = 0}^{4095}\ket{j}\ket{4^j \bmod 35}
	\end{equation}
	上面的的量子态也可以表述成下面的形式
	\begin{equation}
		\begin{aligned}
			\varphi &=  \frac{1}{64}((\ket{0}+\ket{6}+\ket{12}+\cdots +\ket{4092})\ket{1}\\
			&+(\ket{1}+\ket{7}+\ket{13}+\cdots +\ket{4093})\ket{4}\\
			&+(\ket{2}+\ket{8}+\ket{14}+\cdots +\ket{4094})\ket{16}\\
			&+(\ket{3}+\ket{9}+\ket{15}+\cdots +\ket{4095})\ket{29}\\
			&+(\ket{4}+\ket{10}+\ket{16}+\cdots +\ket{4090})\ket{11}\\
			&+(\ket{5}+\ket{11}+\ket{17}+\cdots +\ket{4091})\ket{9})
		\end{aligned}
	\end{equation}
	\item 然后对上面的第一个寄存器进行傅里叶逆变化。上面的量子态可以看作是六个态的叠加态，对其中每个态的数据进行傅里叶逆变换可以得到（等价于量子态进行量子傅里叶逆变换）
	\begin{figure}[H]
		\centering
		\includegraphics[scale=0.4]{figures/QFT224}
		\caption{傅里叶逆变换图像}
		\label{fig:qft224}
	\end{figure}
	\item 对第一个量子寄存器进行测量，不妨假设读取得到的概率峰值为数字3414，则依据连分数算法可以得到\begin{equation}
		\frac{3414}{4096}\approx \frac{5}{6}
	\end{equation}
	从而得到正确的周期$r=6$。
\end{itemize}

下面使用pyqpanda给出算法的量子线路部分，其中待分解的数字为15，选取的随机数$a=2$
\lstinputlisting[
style=PythonStyle,
numbers=left,
linewidth=0.94\columnwidth,
xleftmargin=0.06\columnwidth,
basicstyle=\linespread{1} \scriptsize \ttfamily,
caption=\text{Shor 算法示例},
label=code:QPanda_Shor
]{code/2.2/Shor.py}

通过第一个寄存器的测量结果可以读取到四个高概率测量结果
\begin{equation}
	0=\frac{0}{4},\ \frac{1}{4},\ \frac{1}{2}=\frac{2}{4},\ \frac{3}{4}
\end{equation}

例如，运行结果为：\{'c0': False, 'c1': False, 'c2': False, 'c3': False, 'c4': False, 'c5': False, 'c6': True, 'c7': False\}，对应的分数为$\frac{64}{256}=\frac{1}{4}$，从而可以得到
从而得到2的周期4（$2^4\equiv 1 \bmod 15$）。代码\ref{code:QPanda_Shor}所使用的量子线路包含$5n+2$个量子比特，在实际线路中，可以采用多种多样的方式降低比特数，比如序列傅里叶变换（semi-classical quantum
Fourier transform）、傅里叶模数运算组件\cite{beauregard2002circuit}、脏量子比特辅助计算\cite{gidney2017factoring}等多种方式降低线路所需的比特数。

此外，Shor算法还能够高效求解离散对数问题，这意味着椭圆曲线上加法群以及其他有限域上的离散对数问题都能够被大规模量子计算机以多项式时间复杂度解决。但是这部分内容需要更多的数学预备知识，实现的线路也远比代码\ref{code:QPanda_Shor}复杂，这里不再展开，有兴趣的读者可以参考\cite{roetteler2017quantum,nielsen2002quantum,aono2022present}。

\begin{exercise}
	尝试利用连分数算法由上例中的$\frac{3414}{4096}$得到目标$\frac{5}{6}$。
\end{exercise}

\begin{exercise}
	开放问题：尽管对于椭圆曲线加法群或者一般有限域的量子线路的构造是困难的，但$\mathbb{Z}/p\mathbb{Z}$上的结构足够简单，其上的离散对数问题是不需要借助额外接口就能够使用pyqpanda求解的，并且求解线路与整数分解问题的线路是相近的。请仿照\ref{code:QPanda_Shor}给出离散对数问题求解的量子线路部分，设待求解的问题为$$3^x\equiv 2 \bmod 7$$
\end{exercise}


